Interpretable Neuron Structuring with Graph Spectral Regularization

While neural networks are powerful approximators used to classify or embed data into lower dimensional spaces, they are often regarded as black boxes with uninterpretable features. Here we propose Graph Spectral Regularization for making hidden layers more interpretable without significantly impacting performance on the primary task. Taking inspiration from spatial organization and localization of neuron activations in biological networks, we use a graph Laplacian penalty to structure the activations within a layer. This penalty encourages activations to be smooth either on a predetermined graph or on a feature-space graph learned from the data via co-activations of a hidden layer of the neural network. We show numerous uses for this additional structure including cluster indication and visualization in biological and image data sets.

==> figures/cartoon.tex <==
\begin{figure}[ht]
    \begin{center}
    \includegraphics[width = 0.5\linewidth]{figures/cartoon_v3.png}
    \end{center}
    \caption{(a) Enforcing graph structure (in this case a ring), adds a penalty of $z^T L z$ for some activation vector $z$ and fixed Laplacian matrix $L$. (b) Learning graph structure alternates between learning a graph structure from the activations of the hidden layer $z$ and training the autoencoder with a regularization penalty over the learned graph encouraging smoothness over the graph.}
    \label{fig:cartoon}
\end{figure}
\vspace{-2.5mm}

==> neuron_graph_layer.tex <==
%Consider a given layer in an artificial neural network, and let $\mathcal{V} = \{\nu_1, \ldots, \nu_n\}$ be the neurons in this layer. These neurons can essentially be regarded as functions of inputs to the neural network, and map each input to an $n$ dimensional vector $\boldsymbol{\nu}(x) = [\nu_1(x), \ldots, \nu_n(x)]^T \in \mathbbm{R}^n$. Typically, no particular structure is being directly imposed on the range of $\boldsymbol{\nu}$ beyond general notions of bounded $L_p$ norm (e.g., Euclidean $L_2$ norm or $L_1$ norm as a proxy for sparsity). This is clear with fully connected layers, but even with convolutional ones that introduce some relation between neurons within each layer, there is still no clear topological structure for the representations obtained by the entire layer as a whole. Indeed, convolutional layers typically learn multiple channels (or filters) from input signals, and while neurons within each channel can be organized in spatiotemporal coordinates, there are no imposed relations between the different channels.

%Since many applications of neural networks essentially focus on supervised learning tasks (whether predictive or generative), where hidden layer neurons are only used as intermediate computational units, their unstructured nature is not considered an important issue. However, when using neural networks for unsupervised and exploratory tasks, in which the hidden layers are treated as latent data representations, their lack of structure makes the interpretation of the resulting representations challenging if not impossible. To address this challenge, autoencoders and similar unsupervised deep models typically restrict their bottleneck layer to have two or three neurons, thus mapping data points to $\mathbbm{R}^2$ or $\mathbbm{R}^3$, where the entire data can be visualized as a 2D or 3D cloud of points. While this approach is useful for getting a general understanding of structures (e.g., clustering or trends) in the data, it significantly limits the amount of information that can be captured by such latent representations. Furthermore, it underutilizes the ability of a human observer to identify rich patterns in 2D displays. Indeed, human perception in natural settings is not tuned to observe particle clouds, but rather to recognize shapes, identify textures, and assess relative sizes of objects. Such elements are often used by visualization techniques in various fields, such as TreeMap~\citep{shneiderman1992treemaps}, audio spectrograms~\citep{flanagan1972speech}, and even classic box plots and histograms~\citep{tukey1977exploratory}.   

% Here, we propose a new approach for producing human interpretable patterns in the latent representation obtained by hidden layers of neural networks. To this end, we impose a graph topology on the neurons in $\mathcal{V}$. 

%Formally, we consider the neurons $\mathcal{V}$ as vertices of a graph with weighted edges between them defined by an $n \times n$ adjacency matrix $W$. Then, for any given input $x$ to the network, we consider the activations $[\nu_1(x), \ldots, \nu_n(x)]$ as a signal $\boldsymbol{\nu}$ over this neuron graph. We propose here to utilize this graph signal structure of a neural network layer by considering graph signal processing notions, we can define spectral regularizations that control the regularity or smoothness of learned signals, as explained in Section~\ref{sec:spec_reg}. %Second, by utilizing sparse graph wavelet dictionaries, we can define a new type of bottleneck that forces autoencoder middle layers to encode inputs by sparse set of localized dictionary atoms (e.g., as done in compressive sensing and dictionary learning), as explained in Section~\ref{sec:spec_bottleneck}. 
%Second, by utilizing simple graph structures, such as a ring graph or a 2D lattice we can force downstream layers to be convolutional layers, regardless of whether the input of the network was structured or not. Section~\ref{sec:results} demonstrates the utility of each of these design choices for several data exploration applications, in both supervised and unsupervised settings.

% \subsection{Spectral graph regularization}
% \label{sec:spec_reg}

\input{spectral_regularization}

==> spectral_regularization.tex <==
\section{Laplacian Smoothing Regularization} 

Given the Fourier coefficients $\widehat{\boldsymbol{\nu}}$, we can phrase regularization penalties
$$
\|\widehat{\boldsymbol{\nu}}(x)\|_{L_2(\boldsymbol{\mu})}^2 = \sum_{j=0}^{n-1} \boldsymbol{\mu}(\lambda_j) \left( \widehat{\boldsymbol{\nu}}_{(x)}[j] \right)^2
$$
that penalize portions of the graph spectrum, determined by $\boldsymbol{\mu}$, which acts as a graph filter. In particular, by setting $\boldsymbol{\mu}$ to be a high-pass filter, we can penalize high frequency, and thus encourage smooth latent representations (over the neuron graph sense). A natural choice for such weights is to simply set them by the identity $\boldsymbol{\mu}(\lambda_j) = \lambda_j$, which results in a penalty term that can be rewritten as the the quadratic form 
$$
[\boldsymbol{\nu}(x)]^T \mathbf{L} \boldsymbol{\nu}(x) = \sum_{j=0}^{n-1} \lambda_j \left( \widehat{\boldsymbol{\nu}}_{(x)}[j] \right)^2 ,
$$
and thus be computed directly from the activation signal without eignedecomposition of the graph Laplacian. This regularization has been proposed in various forms in the graph signal processing literature~\citep[see, e.g.,][] {belkin2004regularization, zhou2004regularization, shuman2013emerging}, and to it here as Laplacian smoothing regularization and demonstrate its utility for producing interpretable latent representations in hidden layers of neural networks in Section~\ref{sec:results}. We also note that more generally, since our regularization here is based in weighted $L^2$ norm of the Fourier coefficients, any polynomial filter can be rewritten directly as polynomials of the Laplacian (i.e., without requiring eigendecomposition), and thus the notion of spectral regularization can be further generalized to emphasize other portions of the spectrum. However, such generalization is beyond the scope of this paper, and is left for future work.

==> zzz_old.tex <==
\author{Alexander Tong\footnotemark[1] \\
%Department of Computer Science \\
Yale University \\
%New Haven, CT 06511 \\
\texttt{alexander.tong@yale.edu} \\
\And
David van Dijk\thanks{These authors contributed equally} \\
Departments of Genetics \\
Yale University \\
%New Haven, CT 06510 \\
\texttt{david.vandijk@yale.edu} \\
\And
Jay S. Stanley III\\
Computational Biology \& Bioinformatics Program \\
Yale University \\
%New Haven, CT 06510 \\
\texttt{jay.stanley@yale.edu} \\
\And
Matthew Amodio\\
Department of Computer Science\\
Yale University \\
New Haven, CT 06510 \\
\texttt{matthew.amodio@yale.edu} \\
\And
Guy Wolf\footnotemark[2]\\
Applied Mathematics Program \\
Yale University \\
New Haven, CT 06511 \\
\texttt{guy.wolf@yale.edu}\\
\And
Smita Krishnaswamy\thanks{These authors contributed equally;~~{\small \Letter} Corresponding author}~~~{\normalfont\small \Letter} \\
Departments of Genetics \& Computer Science\\
Yale University \\
New Haven, CT 06510, USA \\
\texttt{smita.krishnaswamy@yale.edu}\\
}


%\subsection{Enforcing Standard Graph Topologies}
%\label{sec:results:enforcing}
%Often it is useful to extract a known structure from a dataset. Here we show how to extract progression using a ring graph, hierarchies using a clustered graph, and visual features using a 2d lattice graph. We note that the regularization coefficient that controls the balance in our loss function between reconstruction and smoothness is dataset dependent and a number of settings must be tried. There cannot be a universal regularization coefficient across all datasets as the regularization operates on a different layer of the network than reconstruction, the relative network weight scales (which are sensitive to initialization) affect the parameter setting.

%Here we demonstrate graph regularization on a variety of datasets using predetermined graph structures. In each case we show the increased interpretability offered by the graph in terms of data topology and feature abstraction.  

%\input{figures/teapot.tex}
%\paragraph{Enforcing Ring Graph Structure}
%First, in Figure~\ref{fig:teapot} we demonstrate regularization using a standard ring graph. Although it may not be clear what graph the features should take in the original space, we can often surmise an overall topology of the examples. Here we have the rotating teapot dataset~\cite{weinberger2004learning}. This dataset is comprised of 400 images of a teapot rotating one full circle around the vertical axis. There is a ring topology here as images that are very close rotations of each other should be represented similarly in the autoencoder. We train a graph spectral regularized autoencoder on the first 100 PCA components of these images with mean squared error (MSE) and graph spectral regularization at different coefficients balancing MSE and our regularization. Without regularization it is not clear that there are repeated structures on the graph. However, with higher regularization coefficients we can see the smoothness along the line and the symmetries of the teapot are more apparent. For example, the spout and the handle of the teapot look very similar (in a MSE sense) so when the teapot has the handle on the left looks similar to when the handle is on the right. This is apparent in the right most plot as the two bright white spots on the embedding heatmap.

%\subsection{Hierarchical Structure}

%Finally, we look at hierarchical structure, First we show that if we would like to capture a structure known apriori, for example we are given information that there are X distinct cell types, or X clusters in the data that we would like to examine further, then we can do so by constructing the appropriate graph. If for example we know that there should be 5 clusters of the data then we can form a graph with 5 disconnected complete subgraphs. Finally, we show that we can learn this hierarchical structure in a developing neuron dataset without prior knowledge on the number of clusters.
